Theoretical aspects of quantum electrodynamics in a finite volume with periodic boundary conditions

First-principles studies of strongly-interacting hadronic systems using lattice quantum chromodynamics (QCD) have been complemented in recent years with the inclusion of quantum electrodynamics (QED). The aim is to confront experimental results with more precise theoretical determinations, e.g. for the anomalous magnetic moment of the muon and the CP-violating parameters in the decay of mesons. Quantifying the effects arising from enclosing QED in a finite volume remains a primary target of investigations. To this end, finite-volume corrections to hadron masses in the presence of QED have been carefully studied in recent years. This paper extends such studies to the self-energy of moving charged hadrons, both on and away from their mass shell. In particular, we present analytical results for leading finite-volume corrections to the self-energy of spin-0 and spin-$\frac{1}{2}$ particles in the presence of QED on a periodic hypercubic lattice, once the spatial zero mode of the photon is removed, a framework that is called $\mathrm{QED}_{\mathrm{L}}$. By altering modes beyond the zero mode, an improvement scheme is introduced to eliminate the leading finite-volume corrections to masses, with potential applications to other hadronic quantities. Our analytical results are verified by a dedicated numerical study of a lattice scalar field theory coupled to $\mathrm{QED}_{\mathrm{L}}$. Further, this paper offers new perspectives on the subtleties involved in applying low-energy effective field theories in the presence of $\mathrm{QED}_{\mathrm{L}}$, a theory that is rendered non-local with the exclusion of the spatial zero mode of the photon, clarifying recent discussions on this matter.

==> sections/sumintdiff.tex <==
% !TEX root = ../sefv.tex !TEX spellcheck = en-US
%============================================================================
\subsection{Standard sum-integral difference}
Let $f$ be a smooth, rapidly decreasing function on $\R^d$ (in the Schwartz
sense). Such a function is integrable and  the sum-integral difference can be unambiguously defined
\begin{equation}
    \Delta_nf(n)=\sum_{n\in\Z^d}f(n)-\int\diff^d n\,f(n)\,.
\end{equation}
The symbol $\Delta_n$ defines a linear operator on the space of such
functions. Using the Poisson summation formula, one obtains
\begin{equation}
    \Delta_nf(n)=\sump_{m\in\Z^d}\hat{f}(m)\,,\label{eq:psf}
\end{equation}
where the Fourier transform $\hat{f}$ is defined by
\begin{equation}
    \hat{f}(m)=\int\diff^d n\,f(n)e^{-2\pi im\cdotp n}\,.
\end{equation}
In the quantum field theory applications considered here, the function $f$ will
represent the expression for some momentum-space Feynman diagram and will not be
integrable in the presence of ultraviolet divergences. However, non-integrable
functions which grow slower than a given power have a Fourier transform defined
as a tempered distribution. In this context, the right-hand side
of~\cref{eq:psf} extends unambiguously to non-integrable functions
if the singular support of $\hat{f}$ does not contain any $m\in\Z^d$ for $m\neq
0$ (\ie the terms $\hat{f}(m)$ in the sum correspond to well-defined numbers)
and the sequence $\hat{f}(m)$ decays fast enough so that the series
$\sum_m'\hat{f}(m)$ converges.

A direct first application of this general definition is the cancellation of the
sum-integral difference of a polynomial $P(n)$ in the components of $n$
\begin{equation}
    \Delta_n P(n)=0\,.
\end{equation}
Indeed, the Fourier transform $\hat{P}(m)$ is a polynomial in derivatives of
delta functions $\delta(m_j)$ and the sum in~\cref{eq:psf} is trivially zero. A
more realistic example can be constructed with a propagator-like function
\begin{equation}
    f(n)=\frac{1}{(n^2+\mu^2)^{\alpha}}\,,\label{eq:proplikefn}
\end{equation}
which has the Fourier transform
\begin{equation}
    \hat{f}(m)=\frac{2\pi^{\frac{\alpha}{2}}}{\Gamma(\frac{\alpha}{2})}
    \left(\frac{|m|}{\mu}\right)^{\frac{\alpha-d}{2}}
        \mathrm{K}_{\frac{d-\alpha}{2}}(2\pi|m|\mu)\,,
\end{equation}
where $\mathrm{K}_j$ is the Bessel function of the second kind. Clearly
$\hat{f}(m)$ is smooth and decays exponentially fast for $|m|>0$ and therefore
$\Delta_nf(n)$ is a well defined number.

Typically in finite-volume problems we study how fast a Riemann sum converges to
an integral
\begin{equation}
    \lim_{\eta\to 0}\eta^d\sum_{n\in\Z^d}f(\eta n)=\int\diff^dn\,f(n)\,,
\end{equation}
for $\eta>0$, which can be rewritten as the convergence to zero of the
sum-integral difference
\begin{equation}
    \lim_{\eta\to 0}\eta^d\Delta_nf(\eta n)=0\,.
\end{equation}
Using~\cref{eq:psf}, one gets
\begin{equation}
    \eta^d\Delta_nf(\eta n)=\sump_{m\in\Z^d}\hat{f}\left(\frac{m}{\eta}\right)\,.
    \label{eq:fvmath}
\end{equation}
If $\hat{f}$ is a smooth, rapidly decreasing function then the sum in this last
expression will be dominated by the $|m|=1$ terms. For example
using~\cref{eq:proplikefn},
\begin{equation}
    \eta^d\Delta_nf(\eta n)\underset{\eta\to 0}{\sim}
    \frac{4\pi^{\frac{\alpha}{2}}d}{\Gamma(\frac{\alpha}{2})}
    \left(\frac{\eta}{\mu}\right)^{\frac{\alpha-d}{2}}
    e^{-2\pi\eta\mu}\,,\label{eq:fvmassive}
\end{equation}
which is a version of the known result of the exponential decay of finite-volume
effects on a massive off-shell diagram.

All the cases studied here relied on the fast decay of $\hat{f}(m)$
in~\cref{eq:psf}. If $f$ is a smooth function then typically $\hat{f}(m)$ decays
faster than any power of $|m|$. In field theory this typically happens when $f$
has real singularities. Even then~\cref{eq:psf} might still be well-defined. But
typically the convergence of~\cref{eq:fvmaster} will only follow a power law and
will not be rapidly decreasing like in~\cref{eq:fvmassive}. This is what happens
for example in finite-volume effects to on-shell amplitudes [REF]. In
finite-volume periodic QED this sum typically diverges as a consequence of the
$n=0$ photon singularity in $f(n)$. This is another way to motivate the
construction of $\qedl$ that was discussed in~\cref{sec:qedl}. In the next
section we discuss modified sum-integral differences for finite-volume effects
in $\qedl$.
%============================================================================
\subsection{$\qedl$ sum-integral difference}
\todo{(AP) finish this or forget entirely about this appendix}

